Functional Information, Optimal Channel Simulation and Lossy Source Coding

We characterize, within a constant number of bits, the minimum achievable rate for several one-shot coding problems, such as channel simulation and lossy source coding. The basis of our work is a new information measure between random variables $X, Y$ that we call the functional information $I_F(X \to Y)$. We show that this quantity characterizes the minimum one-shot rate $R^*(X \to Y)$ of channel simulation, in which a sample $Y \sim P_{Y \mid X}$ is communicated in the presence of common randomness: $I_F(X \to Y) \leq R^*(X \to Y) < I_F(X \to Y) + 1.45$. For the achievability result, we construct an explicit code using the Poisson functional representation. Using these results, we develop new bounds for one-shot variable-rate lossy source coding: given some distortion measure $\Delta$, we use $I_F(X \to Y)$ to define the functional rate-distortion function $R_F$. Then, letting $R_O$ denote the one-shot operational rate-distortion function with private encoder randomness and distortion measure $\Delta$, we make use of our channel simulation result to show that $R_F(D) \leq R_O(D) < R_F(D) + 2.45$ at every positive distortion level $D$. Finally, we generalize our channel simulation result by introducing the R\'enyi $\alpha$-functional information $I_{F, \alpha}(X \to Y)$ and show that it characterizes the minimum Arimoto-R\'enyi conditional entropy for channel simulation, ${R^*_\alpha(X \to Y)}$, associated with the Campbell cost: ${I_{F, \alpha}(X \to Y) \leq R^*_{\alpha}(X \to Y) \leq I_{F, \alpha}(X \to Y) + c_\alpha}$, where $c_\alpha$ is a constant depending on $\alpha \in (0, 1)$.

==> img/binary_approximate.tex <==
\pgfmathdeclarefunction{Hb}{1}{%
  \pgfmathparse{-(#1*ln(#1)+(1-#1)*ln(1-#1))/ln(2)}%
}

\newcommand{\ChannelPlot}[3]{%
\begin{tikzpicture}
\begin{axis}[
    width=0.5\textwidth,
    height=0.3\textwidth,
    xmin=0, xmax=0.5,
    ymin=0, ymax=0.6,
    axis x line=bottom,
    axis y line=left,
    grid=none,
    tick align=outside,
    xlabel={$\epsilon$}
]
\addplot[tabblue, thick]
coordinates {
    (0,{Hb(#1)*abs(#2-#3)})
    (0.5,{Hb(#1)*abs(#2-#3)})
};

\addplot[tabred, thick]
coordinates {
    (0,{Hb((1-#1)*#2+#1*#3)-(1-#1)*Hb(#2)-#1*Hb(#3)})
    (0.5,{Hb((1-#1)*#2+#1*#3)-(1-#1)*Hb(#2)-#1*Hb(#3)})
};

\addplot[black, very thick]
coordinates {
    (0,{Hb(#1)*abs(#2-#3)})
    ({min(#1,1-#1)*abs(#2-#3)},0)
    (0.5,0)
};
\end{axis}
\end{tikzpicture}

\vspace{0.25em}

\begin{center}
\begin{tikzpicture}
\node[inner sep=2pt, font=\small] {
\begin{tabular}{@{}c@{\hspace{2pt}}l@{\hspace{0.65cm}}c@{\hspace{2pt}}l@{\hspace{0.65cm}}c@{\hspace{2pt}}l@{}}
\raisebox{0.6ex}{\tikz{\draw[thick, tabblue] (0,0) -- (0.6,0);}} &
$\FI{X}{Y}$ &
\raisebox{0.6ex}{\tikz{\draw[thick, tabred] (0,0) -- (0.6,0);}} &
$\MI{X}{Y}$ &
\raisebox{0.6ex}{\tikz{\draw[very thick, black] (0,0) -- (0.6,0);}} &
$R_F(\epsilon)$
\end{tabular}
};
\end{tikzpicture}
\end{center}
}

\ChannelPlot{0.50}{0.2}{0.75}
